Power-Law Wrinkling Turbulence-Flame Interaction Model for Astrophysical Flames

We extend a model for turbulence-flame interactions (TFI) to consider astrophysical flames with a particular focus on combustion in type Ia supernovae. The inertial range of the turbulent cascade is nearly always under-resolved in simulations of astrophysical flows, requiring the use of a model in order to quantify the effects of subgrid-scale wrinkling of the flame surface. We provide implementation details to extend a well-tested TFI model to low-Prandtl number flames for use in the compressible hydrodynamics code FLASH. A local, instantaneous measure of the turbulent velocity is calibrated for FLASH and verification tests are performed. Particular care is taken to consider the relation between the subgrid rms turbulent velocity and the turbulent flame speed, especially for high-intensity turbulence where the turbulent flame speed is not expected to scale with the turbulent velocity. Finally, we explore the impact of different TFI models in full-star, three-dimensional simulations of type Ia supernovae.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

%\RequirePackage{bm}
\RequirePackage{amssymb}
\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}

% end vectors.tex

